Data Augmentation for Continual RL via Adversarial Gradient Episodic Memory

Data efficiency of learning, which plays a key role in the Reinforcement Learning (RL) training process, becomes even more important in continual RL with sequential environments. In continual RL, the learner interacts with non-stationary, sequential tasks and is required to learn new tasks without forgetting previous knowledge. However, there is little work on implementing data augmentation for continual RL. In this paper, we investigate the efficacy of data augmentation for continual RL. Specifically, we provide benchmarking data augmentations for continual RL, by (1) summarising existing data augmentation methods and (2) including a new augmentation method for continual RL: Adversarial Augmentation with Gradient Episodic Memory (Adv-GEM). Extensive experiments show that data augmentations, such as random amplitude scaling, state-switch, mixup, adversarial augmentation, and Adv-GEM, can improve existing continual RL algorithms in terms of their average performance, catastrophic forgetting, and forward transfer, on robot control tasks. All data augmentation methods are implemented as plug-in modules for trivial integration into continual RL methods.

==> content/acknowledgements.tex <==
% Acknowledgements should only appear in the accepted version.
\section*{Acknowledgements}

\textbf{Do not} include acknowledgements in the initial version of
the paper submitted for blind review.

If a paper is accepted, the final camera-ready version can (and
probably should) include acknowledgements. In this case, please
place such acknowledgements in an unnumbered section at the
end of the paper. Typically, this will include thanks to reviewers
who gave useful comments, to colleagues who contributed to the ideas,
and to funding agencies and corporate sponsors that provided financial
support.

==> content/discussion.tex <==
\section{Discussion}
% \mf{New methods for CRL, like memory mechnism and automatic DA.}

% \mf{Theoretical Guarantees}
\textbf{How to obtain more effective data augmentation for continual RL?} Our paper shows that by incorporating powerful inductive biases, data augmentation, can actually increase the performance of continual RL. But the sequence and the difficulty of tasks may vary in reality, the adaptive and effective data augmentation methods are needed. In our opinion, following the memory-based method \citep{guo2020improved}, the stored data can be used to help generate adaptive augmented data for each task. For task-agnostic continual RL, if there is no clear task delineation, it will be hard for continual learning. Bayesian estimation methods could be a direction like \citep{xu2020task}. 


\textbf{How to justify the effectiveness of data augmentation?}  Although data augmentation has shown great improvement of performance in the continual RL, the reason behind the empirical result is still unknown. In RL, \citep{kostrikov2020image} clarified the effectiveness of data augmentation. However, how data augmentation helps continual RL is still unclear. And the change of data distribution for each task after data augmentation needs to be more clearly demonstrated. In the future, a theoretical framework needs to be established for understanding data augmentation, which will lead to more
theoretically grounded applications of data augmentation for continual RL.  

==> content/related.tex <==
\section{Related Work}

\subsection{Continual Learning background}


\subsection{Data Augmentation}


% One natural way to make training and testing data more similar is data augmentation \cite{kostrikov2020image, 2111.09794, 2004.14990, sinha2022s4rl}.
% By regularizing the model to have the same output for different augmented data points, data augmentation can enforce the agent to learn the invariant representation features. 
% Most of the papers are focused on image-based RL on DeepMind Control suit. Like DrQ \cite{kostrikov2020image}, RAD \cite{2004.14990}, UCB-DrAC \cite{raileanu2020automatic}, SVEA \cite{hansen2021stabilizing}. They use rotation, crop, translation to transform the image.

% Besides augmentation on image-based RL, for state-based RL, \cite{sinha2022s4rl} propose S4RL for the function approximation of the Q-networks.


\subsection{Adversarial Attack}
The literature on adversarial attack \cite{goodfellow2014explaining, madry2017towards, croce2020reliable} is quite closed to this work, with the same idea to devise training process to enhance the robustness of the model. As the first well-known work, the Fast Gradient Sign Method (FGSM) \cite{goodfellow2014explaining} generated imperceptible perturbations by calculating the first-order gradient within $\epsilon$-ball, also with several variations \cite{kurakin2016adversarial, tramer2017space}. Later, \cite{madry2017towards} proposed the Projected Gradient descent (PGD) and achieved significantly adversary, which is a very powerful method not only in adversarial attack but also adversarial training. Additionally, considering the unsupervised domain adaptation problem, \cite{9528987} investigated from adversarial attack perspective and tackle the divergence-agnostic adaptive learning problem, which has few similarities with our work.

To penalize the differences between  between the original and the adversarial examples, adversarial training paradigm was developed, like \cite{sinha2017certifying, madry2017towards, heinze2017conditional}. \cite{sinha2017certifying} proposed an unified adversarial training architecture, by maximizing the worst-case data distribution while optimizing the model parameters with respect to the adversarial examples. Developed from it, \cite{10.5555/3327345.3327439} imposed the constraint in the semantic space, aiming to learn models that are resistant to out-of-distribution samples. 

Adversarial attack also has shown its effectiveness on RL. In \cite{huang2017adversarial}, they obtained the adversarial examples by directly using FGSM \cite{goodfellow2014explaining} to perturb each image at every time step for RL. 
Further, relying on the sequential decision-making property of RL, \cite{lin2017tactics} propose strategically-attack that attacking RL agent at critical moments will be more efficient, and enchanting-attack maliciously luring an agent to a certain state.


However, our work consider to add the adversarial attack examples into the data augmentation process, to help the policy update of continual reinforcement learning.
